Why am I seeing this: Democratizing End User Auditing for Online Content Recommendations

Personalized recommendation systems tailor content based on user attributes, which are either provided or inferred from private data. Research suggests that users often hypothesize about reasons behind contents they encounter (e.g., "I see this jewelry ad because I am a woman"), but they lack the means to confirm these hypotheses due to the opaqueness of these systems. This hinders informed decision-making about privacy and system use and contributes to the lack of algorithmic accountability. To address these challenges, we introduce a new interactive sandbox approach. This approach creates sets of synthetic user personas and corresponding personal data that embody realistic variations in personal attributes, allowing users to test their hypotheses by observing how a website's algorithms respond to these personas. We tested the sandbox in the context of targeted advertisement. Our user study demonstrates its usability, usefulness, and effectiveness in empowering end-user auditing in a case study of targeting ads.

==> content/a0-substitution_impact.tex <==
\clearpage
\appendix

\section{Result of the Impact of Persona Substitution}
\label{appendix: persona substitution}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Different_persona.png}
    \caption{\revise{Comparison of Ad-Attribute Alignment Scores for Different Personas. Single asterisk (*) denote p<0.1, while double asterisks (**) indicate p<0.05.}}
    \Description{This figure presents a series of bar charts comparing Ad-Attribute Alignment Scores across various personas categorized by Age, Gender, Location, Income, and Education Level over three rounds. Each chart shows three groups within a category, highlighting differences in scores. Across all categories, noticeable trends emerge, such as older individuals, females, rural residents, high-income earners, and those with higher education levels generally achieving higher alignment scores. Statistical significance is marked, with a single asterisk (*) denoting p < 0.1 and double asterisks (**) indicating p < 0.05, emphasizing meaningful differences between groups.}
    \label{fig: different persona}
\end{figure}
\clearpage

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/Similar_persona.png}
    \caption{\revise{Comparison of Ad-Attribute Alignment Scores for Similar Personas}}
    \Description{This figure presents a series of bar charts comparing median ad-attribute alignment scores across three rounds for personas with varying demographic attributes: age, gender, location, income, and education level. For age, scores show slight decreases for the young and old groups, while mid-aged personas have fluctuating scores. In gender, male and non-binary personas show consistent scores, while female personas experience a slight dip in Round 3. Location shows marginal score increases for urban personas, stability for suburban personas, and slight decreases for those in the countryside. Income personas demonstrate a small increase for low-income groups, steady scores for medium-income, and a noticeable rise for high-income groups in Round 3. Lastly, education level scores fluctuate slightly for low education, increase for medium education, and show a noticeable rise for high education personas in Round 2. Each chart is color-coded by round, with scores ranging from 0 to 100.}
    \label{fig: similar persona}
\end{figure}

\clearpage
